Almost Tight L0-norm Certified Robustness of Top-k Predictions against Adversarial Perturbations

Top-k predictions are used in many real-world applications such as machine learning as a service, recommender systems, and web searches. $\ell_0$-norm adversarial perturbation characterizes an attack that arbitrarily modifies some features of an input such that a classifier makes an incorrect prediction for the perturbed input. $\ell_0$-norm adversarial perturbation is easy to interpret and can be implemented in the physical world. Therefore, certifying robustness of top-$k$ predictions against $\ell_0$-norm adversarial perturbation is important. However, existing studies either focused on certifying $\ell_0$-norm robustness of top-$1$ predictions or $\ell_2$-norm robustness of top-$k$ predictions. In this work, we aim to bridge the gap. Our approach is based on randomized smoothing, which builds a provably robust classifier from an arbitrary classifier via randomizing an input. Our major theoretical contribution is an almost tight $\ell_0$-norm certified robustness guarantee for top-$k$ predictions. We empirically evaluate our method on CIFAR10 and ImageNet. For instance, our method can build a classifier that achieves a certified top-3 accuracy of 69.2\% on ImageNet when an attacker can arbitrarily perturb 5 pixels of a testing image.

==> impact.tex <==
\section*{Broader Impact}
Adversarial perturbation is one of the biggest security challenges for deploying machine learning in security and safety critical domains such as military applications, precision healthcare, and self-driving cars. Our work studies certified robustness of  smoothed classifiers and can provably secure machine learning in such critical domains. 



==> practice.tex <==
\section{Certification in Practice}
\label{compute_radius}





Given a base classifier $f$, an example $x$, a label $l$, and a   parameter $e$, we aim to compute the certified radius $r_{l}$. 
Our certified radius relies on the probability bounds $\underline{p_l}$ and  $\overline{p}_{\Upsilon_{t}}$, and requires to solve the optimization problem in Equation~\ref{equation_2_solve_to_find_rl}. In particular, we  leverage a Monte Carlo method developed in~\cite{jia2020certified} to estimate $\underline{p_l}$ and $\overline{p}_{\Upsilon_{t}}$ with probabilistic guarantees. 
Moreover, given probability bounds $\underline{p_l}$ and $\overline{p}_{\Upsilon_{t}}$, we use binary search to solve Equation~(\ref{equation_2_solve_to_find_rl}) to find certified radius $r_l$. 

\myparatight{Estimating $\underline{p_l}$ and $\overline{p}_{\Upsilon_{t}}$} 
The probabilities 
$p_1, p_2, \cdots, p_{c}$ 
can be viewed as a multinomial distribution over the label set 
$\{1,2,\cdots, c\}$. 
Given $h(\mathbf{x},e)$ as input, $f(h(\mathbf{x},e))$ can be viewed as a sample from the multinomial distribution. Therefore,  estimating $\underline{p_l}$ and $\overline{p}_i$ for $i\neq l$ is essentially a one-sided \emph{simultaneous confidence interval} estimation problem. In particular, we leverage the simultaneous confidence interval estimation method  developed in~\cite{jia2020certified} to estimate these bounds with a confidence level at least $1-\alpha$. 

Specifically, given an example $\mathbf{x}$ and parameter $e$, we randomly subsample $n$ noisy examples, i.e., $\epsilon^1, \epsilon^2, \cdots,\epsilon^n$, from $h(\mathbf{x},e)$.
We denote by $N_i$ the frequency of the label $i$ predicted by the base classifier for the $n$ noisy examples. 
Formally, we have  $N_j = \sum_{j=1}^n \mathbb{I}(f(\epsilon^i)=j)$, where $j \in \{1,2,\cdots,c\}$ and $\mathbb{I}$ is the indicator function. 
According to~\cite{jia2020certified}, we have the following probability bounds with a confidence level at least $1-\alpha$:
\begin{align}
\label{compute_bound_simuem}
 & \underline{p_l }=B\left(\frac{\alpha}{c};n_l,n-n_l+1\right), \overline{p}_{j}=B(1-\frac{\alpha}{c};n_j+1, n-n_i), \  \forall j \neq l,
\end{align}
where $B(q; \xi,\zeta)$ is the $q$th quantile of a beta distribution with shape parameters $\xi$ and $\zeta$.
%Moreover, 
Following~\cite{jia2020certified}, we estimate $\overline{p}_{\Upsilon_{t}}$ as $ \overline{p}_{\Upsilon_{t}}=\min(\sum_{j \in \Upsilon_{t}}\overline{p}_{j}, 1 - \underline{p_l})$.



